NSA: Neuro-symbolic ARC Challenge

The Abstraction and Reasoning Corpus (ARC) evaluates general reasoning capabilities that are difficult for both machine learning models and combinatorial search methods. We propose a neuro-symbolic approach that combines a transformer for proposal generation with combinatorial search using a domain-specific language. The transformer narrows the search space by proposing promising search directions, which allows the combinatorial search to find the actual solution in short time. We pre-train the trainsformer with synthetically generated data. During test-time we generate additional task-specific training tasks and fine-tune our model. Our results surpass comparable state of the art on the ARC evaluation set by 27% and compare favourably on the ARC train set. We make our code and dataset publicly available at https://github.com/Batorskq/NSA.

==> sec/abstract.tex <==
\begin{abstract}
The Abstraction and Reasoning Corpus (ARC) evaluates general reasoning capabilities that are difficult for both machine learning models and combinatorial search methods. 
We propose a neuro-symbolic approach that combines a transformer for proposal generation with combinatorial search using a domain-specific language. 
The transformer narrows the search space by proposing promising search directions, which allows the combinatorial search to find the actual solution in short time.
We pre-train the trainsformer with synthetically generated data.
During test-time we generate additional task-specific training tasks and fine-tune our model. %We generate synthetic tassks to train ourpre-tranin our transformer and finto fine-tune it during test-time.% on taskeOur transformer is trained on synthetic tasks and fine-tuned for each new task via test-time adaptation.
Our results surpass comparable state of the art on the ARC evaluation set by 27\% and compare favourably on the ARC train set.
We make our code and dataset 
\textcolor{red}{publicly accessible link to the code and dataset upon acceptance.}.
\end{abstract}
